Studies of correlations between measurements of jet observables

We present a method for calculation of statistical correlations between measured jet observables in high energy collisions. The method is compared to sampling based methods used in the past. The case of measurements of jet rates in $e^+e^-$ collisions is considered in detail.

==> Makefile <==
#Andrii Verbytskyi, MPI fuer Physik, 2015-2017
latexfile=JetClasses
newname?=JetClasses
STYLE=arxiv

LATEX=latex -halt-on-error -shell-escape
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex
endif

ifeq ($(STYLE),nim)
	STYLE_SPECIFIC_FILES=elsarticle.cls $(latexfile)-nim.tex
endif

ifeq ($(STYLE),jinst)
	STYLE_SPECIFIC_FILES=jinstpub.sty newtxtt.sty $(latexfile)-jinst.tex elsarticle-num.bst
endif


ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex
endif


ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex
endif


all: $(latexfile)-$(STYLE).pdf

tar:  Makefile $(figures) $(constanttables) $(tables) $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
	mkdir -p TAR/Tables
	mkdir -p TAR/ConstantTables
	cp Makefile  $(latexfile).bst $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
	cp $(constanttables) TAR/ConstantTables
	cp $(tables) TAR/Tables
	cp $(figures) TAR/Figures
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

#ifeq ($(STYLE),epjc)
#	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
#	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
#	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
#	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
#endif
	
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -k -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),jinst)
	#####-->A trick to get the bib file for jinst build system
	$(MAKE) -k -C TAR $(newname)-$(STYLE).dvi
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
	rm -rf ConstantTables/Runep*
endif
	rm -rf $(newname).tar.gz
	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -f $(newname).zip
	cd TAR; zip -r ../$(newname).zip  ./*
	rm -rf TAR


figures= \
	Figures/eekt_paths_eesherpa_0.12_91.tex \
	Figures/eekt_rates_eesherpa_0.12_91.tex \
	Figures/eekt_comparison_eesherpa_91.tex \
	Figures/mpantikt_paths_ppsherpa_0.12_7000.tex  \
	Figures/mpantikt_rates_ppsherpa_0.12_7000.tex \
	Figures/mepkt_paths_epsherpa_0.12_55.tex  \
	Figures/mepkt_rates_epsherpa_0.12_55.tex

tables= \
	Tables/constants.txt \
	Tables/eekt_my_eesherpa_0.12_91.tex \
	Tables/eekt_mc_eesherpa_0.12_91.tex \
	Tables/constants_et.txt \
	Tables/mepkt_my_epsherpa_0.12_55.tex \
	Tables/mepkt_transform.tex \
	Tables/constants_pt.txt \
	Tables/mpantikt_my_ppsherpa_0.12_7000.tex \
	Tables/mpantikt_transform.tex


constanttables=ConstantTables/Runeesherpa_0.12.dat ConstantTables/Runepsherpa_0.12.dat ConstantTables/Runppsherpa_0.12.dat


$(latexfile)-$(STYLE).dvi :  $(figures) $(constanttables) $(tables) $(latexfile).bst\
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex   $(STYLE_SPECIFIC_FILES)
	sed -i 's@rotate=-.*]@rotate=-90]@g' Figures/*paths*.tex
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
	sed -i '/digital/d' $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)

$(latexfile)-$(STYLE).pdf : $(latexfile)-$(STYLE).ps
	ps2pdf -dUseCIEColor -dPDFSETTINGS=/printer -sPAPERSIZE=a4  $(latexfile)-$(STYLE).ps $(latexfile)-$(STYLE).pdf

ps : $(latexfile)-$(STYLE).ps 

pdf : $(latexfile)-$(STYLE).pdf
$(latexfile)-$(STYLE).ps : $(latexfile)-$(STYLE).dvi
	dvips -Ppdf -t a4 $(latexfile)-$(STYLE)


$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		cat $$a | aspell  list --add-tex-command="bibliographystyle p"  --add-tex-command="app p" --add-tex-command="label p" --add-tex-command="eq p" --add-tex-command="usetikzlibrary p" --add-tex-command="sect p" --add-tex-command="fig p" --add-tex-command="tab p"  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB ;\
		done

		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-tex-command="bibliographystyle p" --add-tex-command="label p"  --add-tex-command="ltset p" --add-tex-command="usetikzlibrary p" --add-tex-command="sect p" --add-tex-command="fig p" --add-tex-command="tab p"  --add-extra-dicts=./$(latexfile).rws  -t --dont-tex-check-comments -d en_GB -c $$a ;\
		done

clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm


typos:
	for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		cat $$a | grep " \.";\
		cat $$a | grep " \,";\
		cat $$a | grep " \;";\
		cat $$a | grep "a a";\
		cat $$a | grep "the the";\
		cat $$a | grep "of of";\
		cat $$a | grep "for for";\
		done


==> Tables/mepkt_transform.tex <==
\begin{tabular}{|cccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc||c|}\hline
0&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20&21&22&23&24&25&26&27&28&29&30&31&32&33&34&35&36&37&38&39&40&41&42&43&44&45&46&47&48&49&50&51&52&53&54&55&56&57&58&59&60&61&62&63&\\\hline\hline
0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &2 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &3 &0\\
    &0 &0 &0 &1 &1 &1 &1 &2 &2 &2 &2 &3 &3 &3 &3 &0 &0 &0 &0 &1 &1 &1 &1 &2 &2 &2 &2 &3 &3 &3 &3 &0 &0 &0 &0 &1 &1 &1 &1 &2 &2 &2 &2 &3 &3 &3 &3 &0 &0 &0 &0 &1 &1 &1 &1 &2 &2 &2 &2 &3 &3 &3 &3 &1\\
    &    &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &0 &1 &2 &3 &2\\
\hline\end{tabular}


==> Tables/mpantikt_transform.tex <==
\begin{tabular}{|cccccccccccccccccccccccccccccccccccccccccccccccc||c|}\hline
0&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20&21&22&23&24&25&26&27&28&29&30&31&32&33&34&35&36&37&38&39&40&41&42&43&44&45&46&47&\\\hline\hline
0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0\\
    &1 &0 &0 &0 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &0 &0 &0 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1\\
    &    &1 &0 &0 &0 &1 &0 &0 &1 &0 &0 &0 &0 &0 &0 &1 &0 &0 &0 &1 &0 &0 &1 &0 &0 &0 &0 &0 &0 &1 &0 &0 &1 &0 &0 &0 &0 &0 &1 &0 &0 &0 &0 &0 &0 &0 &0 &2\\
    &    &    &1 &0 &0 &0 &1 &0 &0 &1 &0 &1 &0 &0 &0 &0 &1 &0 &0 &0 &1 &0 &0 &1 &0 &1 &0 &0 &0 &0 &1 &0 &0 &1 &0 &1 &0 &0 &0 &1 &0 &1 &0 &0 &1 &0 &0 &3\\
    &    &    &    &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &4\\
    &    &    &    &    &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &5\\
    &    &    &    &    &    &0 &0 &0 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &0 &0 &0 &1 &1 &1 &0 &0 &0 &0 &0 &0 &6\\
    &    &    &    &    &    &    &0 &0 &0 &0 &0 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &0 &0 &0 &0 &1 &1 &0 &1 &1 &0 &7\\
    &    &    &    &    &    &    &    &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &8\\
    &    &    &    &    &    &    &    &    &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &1 &1 &1 &1 &1 &1 &0 &0 &0 &0 &0 &0 &0 &0 &0 &9\\
    &    &    &    &    &    &    &    &    &    &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &1 &1 &1 &0 &0 &0 &10\\
    &    &    &    &    &    &    &    &    &    &    &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &1 &1 &1 &11\\
\hline\end{tabular}

